In Search for an Optimal Authenticated Byzantine Agreement

In this paper, we challenge the conventional approach of state machine replication systems to design deterministic agreement protocols in the eventually synchronous communication model. We first prove that no such protocol can guarantee bounded communication cost before the global stabilization time and propose a different approach that hopes for the best (synchrony) but prepares for the worst (asynchrony). Accordingly, we design an optimistic byzantine agreement protocol that first tries an efficient deterministic algorithm that relies on synchrony for termination only, and then, only if an agreement was not reached due to asynchrony, the protocol uses a randomized asynchronous protocol for fallback that guarantees termination with probability 1. We formally prove that our protocol achieves optimal communication complexity under all network conditions and failure scenarios. We first prove a lower bound of $\Omega(ft+ t)$ for synchronous deterministic byzantine agreement protocols, where $t$ is the failure threshold, and $f$ is the actual number of failures. Then, we present a tight upper bound and use it for the synchronous part of the optimistic protocol. Finally, for the asynchronous fallback, we use a variant of the (optimal) VABA protocol, which we reconstruct to safely combine it with the synchronous part. We believe that our adaptive to failures synchronous byzantine agreement protocol has an independent interest since it is the first protocol we are aware of which communication complexity optimally depends on the actual number of failures.

==> algLeaderBasedView.tex <==

\begin{algorithm}
\caption{Linear LBV parametrized with $sq$ and $leader$:
API for a party $p_i$.} 
\begin{algorithmic}[1]
\footnotesize

\Statex \textbf{Local variables initialization:}
\Statex \hspace*{0.4cm} $S_{\emph{key}} = S_{\emph{lock}} =
S_{\emph{commit}} = \{\}$
\Statex \hspace*{0.4cm} $\textbf{keyProof}, \textbf{lockProof},
\textbf{commitProof} \in (\mathbb{V} \times \{0,1\}^*) \cup\{\bot\}$
with selectors \emph{val} and \emph{proof}, initially $\bot$ 
\Statex \hspace*{0.4cm} $\emph{active} \gets \emph{true}$
; $\emph{done} \gets \emph{false}$

 

\Statex

\Upon{wedgeView($\emph{sq}, \emph{leader}$)
invocation}

	\State $\emph{active} \gets \emph{false}$
	\State return $\lr{\textbf{keyProof}, \textbf{lockProof},
	\textbf{commitProof}}$

\EndUpon

\Statex

\Upon{startView($\emph{sq}, \emph{leader}$) invocation}

\State start processing messages associated with \emph{sq} and
\emph{leader}
\Comment{some of these messages might be already received}
\If{\emph{leader} = $p_i$}
	
	\State \hspace*{1cm} \textcolor{gray}{**//first step//**}
	\State send ``$\textsc{preKeyStep}, sq, leader,
	\emph{VALUE}, \emph{KEY}$'' to all parties
	\State \textbf{wait} until $|S_{\emph{key}}| = n-t$
	\State $\nu_k \gets \emph{threshold-sign}(S_{\emph{key}})$
	
	\State \hspace*{1cm} \textcolor{gray}{**//second step//**}
	\State send ``$\textsc{KeyStep}, sq, leader,
	\emph{VALUE}, \nu_k$'' to all parties
	\State \textbf{wait} until $|S_{\emph{lock}}| = n-t$
	\State $\nu_l \gets \emph{threshold-sign}(S_{\emph{lock}})$
	
	\State \hspace*{1cm} \textcolor{gray}{**//third step//**}
	\State send ``$\textsc{lockStep}, sq, leader,
	\emph{VALUE}, \nu_l$'' to all parties
	\State \textbf{wait} until $|S_{\emph{commit}}| = n-t$
	\State $\nu_c \gets \emph{threshold-sign}(S_{\emph{commit}})$
	
	\State \hspace*{1cm} \textcolor{gray}{**//broadcast the commit//**}
	\State send ``$\textsc{commit}, sq, leader,
	\emph{VALUE}, \nu_c$'' to all parties 

\EndIf

\State \textbf{wait} for $\emph{done} = \emph{true}$
\State return $\lr{\textbf{keyProof}, \textbf{lockProof},
	\textbf{commitProof}}$ 
 
\EndUpon

\Statex





\end{algorithmic}
\label{alg:LBV-API}
\end{algorithm}



\begin{algorithm}
\caption{Linear LBV parametrized with $sq$ and $leader$:
$p_i$'s message handlers.} 
\begin{algorithmic}[1]
\footnotesize


\Receiving{``$\textsc{preKeyStep}, sq, \emph{leader}, \emph{value},
\emph{key}$'' from \emph{leader}}
	\If{\emph{active} $\wedge$ ($\emph{LOCK} = \bot $ $\vee$
	$\emph{key.sq} \geq \emph{LOCK}$)}
	\Comment{key is up-to-date}
	
		\If{$\emph{key} = \bot$ $\vee$
		$\emph{threshold-validate}(\lr{\textsc{preKeyStep}, \emph{key.sq},
		\emph{LEADERS}[\emph{key.sq}], \emph{value}}, \emph{key.proof})$)}
		\Comment{key is valid}
			
			\State $\rho_k \gets \emph{share-sign}_i(\lr{\textsc{preKeyStep},
			sq, \emph{leader}, \emph{value}})$
			 
			\State send ``$\textsc{keyShare}, sq, leader, \rho_k$'' to
			\emph{leader}
		
		\EndIf
	
	\EndIf 

\EndReceiving



\Statex

\Receiving{``$\textsc{keyShare}, sq, leader, \rho_k$'' from party
$p_j$ for the first time}

	\If{$leader = p_i$ $\wedge$
	\emph{share-validate}($\lr{\textsc{preKeyStep}, sq, \emph{leader},
	\emph{VALUE}}, p_j, \rho_k)$}
	\Comment{$\rho_k$ is $p_j$'s valid key share}
	
		\State $S_{\emph{key}} \gets S_{\emph{key}} \cup \rho_k$	

	\EndIf


\EndReceiving

\Statex

\Receiving{``$\textsc{KeyStep}, sq, \emph{leader}, \emph{value},
\nu_k$'' from \emph{leader}}
	\If{\emph{active}
	$\wedge$ $\emph{threshold-validate}(\lr{\textsc{preKeyStep}, sq,
	\emph{leader}, \emph{value}}, \nu_k)$}
	
			\State $\textbf{keyProof} \gets \lr{value, \nu_k}$
			\State $\rho_l \gets \emph{share-sign}_i(\lr{\textsc{KeyStep},
			sq, \emph{leader}, \emph{value}})$
			 
			\State send ``$\textsc{lockShare}, sq, leader, \rho_l$'' to
			\emph{leader}
		
	
	\EndIf 

\EndReceiving

\Statex

\Receiving{``$\textsc{lockShare}, sq, leader, \rho_l$'' from party
$p_j$ for the first time}

	\If{$leader = p_i$ $\wedge$
	\emph{share-validate}($\lr{\textsc{KeyStep}, sq, \emph{leader},
	\emph{VALUE}}, p_j, \rho_l)$}
	
		\State $S_{\emph{lock}} \gets S_{\emph{lock}} \cup \rho_l$	

	\EndIf

\EndReceiving


\Statex

\Receiving{``$\textsc{lockStep}, sq, \emph{leader}, \emph{value},
\nu_l$'' from \emph{leader}}
	\If{\emph{active}
	$\wedge$ $\emph{threshold-validate}(\lr{\textsc{KeyStep}, sq,
	\emph{leader}, \emph{value}}, \nu_l)$}
	
			\State $\textbf{lockProof} \gets \lr{value, \nu_l}$
			\State $\rho_c \gets \emph{share-sign}_i(\lr{\textsc{lockStep},
			sq, \emph{leader}, \emph{value}})$
			 
			\State send ``$\textsc{commitShare}, sq, leader, \rho_c$'' to
			\emph{leader}
		
	
	\EndIf 

\EndReceiving

\Statex

\Receiving{``$\textsc{commitShare}, sq, leader, \rho_c$'' from party
$p_j$ for the first time}

	\If{$leader = p_i$ $\wedge$
	\emph{share-validate}($\lr{\textsc{lockStep}, sq, \emph{leader},
	\emph{VALUE}}, p_j, \rho_c)$}
	
		\State $S_{\emph{commit}} \gets S_{\emph{commit}} \cup \rho_c$	

	\EndIf

\EndReceiving

\Statex

\Receiving{``$\textsc{commit}, sq, \emph{leader}, \emph{value},
\nu_c$'' from \emph{leader}}
	\If{\emph{active}
	$\wedge$ $\emph{threshold-validate}(\lr{\textsc{lockStep}, sq,
	\emph{leader}, \emph{value}}, \nu_c)$}
	
			\State $\textbf{commitProof} \gets \lr{value, \nu_c}$
%  			\State return $\lr{\textbf{key}, \textbf{lock}, \textbf{commit}}$
 			\State $\emph{done} \gets \emph{true}$
		
	
	\EndIf 

\EndReceiving



\end{algorithmic}
\label{alg:LBV-messages}
\end{algorithm}





==> gst.tex <==
\section{Eventual synchrony}
\label{sec:gst}

$O(n^2)$ with $f=t$  -- deterministic after GST or randomized in
asynchrony.

==> optimistic.tex <==
\section{Optimistic Asynchronous Byzantine Agreement}
\label{sec:asynchronous}

Put everything together.




==> related.tex <==
\section{Related Work}
\label{sec:related}

\begin{itemize}
  
  \item Synch Hotstuff and F-BFT
  \item Dolev Strong
  \item Byzantine Agreement with Optimal Early Stopping, Optimal
  Resilience and Polynomial Complexity
  \item VABA
  \item Classic early stopping
  \item Synchronizer
  \item Tell the story of the linear LBV -- ideas from Hotstuff to add
  anther phase that were also used in VABA for a quadratic byzantine
  agreement. Later generalize into the LBV abstraction in ACE. we use
  here a linear implementation of LBV.
  
\end{itemize}
